Process Behaviour: Formulae vs. Tests (Extended Abstract)

Process behaviour is often defined either in terms of the tests they satisfy, or in terms of the logical properties they enjoy. Here we compare these two approaches, using extensional testing in the style of DeNicola, Hennessy, and a recursive version of the property logic HML. We first characterise subsets of this property logic which can be captured by tests. Then we show that those subsets of the property logic capture precisely the power of tests.

==> eptcsdata.tex <==
\providecommand{\firstpage}{31}
\providecommand{\publicationstatus}{S. Fr\"oschle, F.D. Valencia (Eds.): Workshop on\\
Expressiveness in Concurrency 2010 (EXPRESS'10).\\
EPTCS 41, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.41.3}{10.4204/EPTCS.41.3}}

